Learning Latent Fields in Multiobject Tracking

Multiobject tracking using measurements from arrays of wireless sensors is a key task in applications ranging from autonomous navigation to public safety. Many existing methods compress raw complex-valued signals into detections or intensity maps during preprocessing, thereby discarding potentially relevant information about the objects and the propagation environment. We propose a Bayesian framework for multiobject tracking that relates object states to raw complex-valued signals via a physics-based superpositional model. The model combines a physics-based array manifold, such as radar steering vectors or the replica vectors of matched-field processing, with a latent field. This latent field is a family of context-dependent signal-power distributions that captures the effects of the objects and the propagation environment and is shared across objects and time. It is parameterized by a conditional normalizing flow, which is trained during runtime without labeled data by maximizing an evidence lower bound (ELBO) derived from the Bayesian model. Learning and inference are thus coupled in a sequential framework. We evaluate the method in simulation and in real-world radio and acoustic experiments, with spatial scales ranging from meters to kilometers, and show that it outperforms detection-based methods.

==> main-labels.tex <==
% Labels of the main paper, copied from Learning-Aided-TBD-TSP-27-V9.aux with the prefix M-,
% as \externaldocument[M-]{Learning-Aided-TBD-TSP-27-V9} of the xr package would define them.
\makeatletter
\newlabel{M-sec:introduction}{{I}{1}}
\newlabel{M-fig:scene}{{1}{1}}
\newlabel{M-sec:method}{{III}{3}}
\newlabel{M-sec:problem}{{\unhbox \voidb@x \hbox {III-A}}{3}}
\newlabel{M-sec:superposition}{{\unhbox \voidb@x \hbox {III-B}}{3}}
\newlabel{M-eq:meas_model}{{1}{3}}
\newlabel{M-eq:rho_gamma}{{2}{3}}
\newlabel{M-tab:complexity_example}{{I}{4}}
\newlabel{M-eq:gauss_lik}{{3}{4}}
\newlabel{M-eq:covariance}{{4}{4}}
\newlabel{M-sec:latent_field_prior}{{\unhbox \voidb@x \hbox {III-C}}{4}}
\newlabel{M-eq:latent_random_field}{{5}{4}}
\newlabel{M-eq:latent_field_evaluation}{{6}{4}}
\newlabel{M-eq:latent_field_power}{{7}{4}}
\newlabel{M-eq:latent_field_prior}{{8}{4}}
\newlabel{M-eq:phi-mixture}{{9}{4}}
\newlabel{M-eq:cond_equals_field}{{10}{4}}
\newlabel{M-eq:field_fdd}{{11}{4}}
\newlabel{M-fig:flow}{{2}{5}}
\newlabel{M-sec:flow}{{\unhbox \voidb@x \hbox {III-D}}{5}}
\newlabel{M-eq:flow_gamma}{{13}{5}}
\newlabel{M-eq:flow_field}{{14}{5}}
\newlabel{M-sec:inference_learning}{{IV}{5}}
\newlabel{M-eq:bayes}{{15}{5}}
\newlabel{M-eq:marg}{{16}{5}}
\newlabel{M-eq:pred_x}{{17}{6}}
\newlabel{M-eq:pred_eta}{{18}{6}}
\newlabel{M-eq:joint_prior}{{19}{6}}
\newlabel{M-fig:vb}{{3}{6}}
\newlabel{M-sec:Var}{{\unhbox \voidb@x \hbox {IV-B}}{6}}
\newlabel{M-eq:frame_objective}{{21}{6}}
\newlabel{M-eq:objective}{{22}{6}}
\newlabel{M-sec:experiments}{{V}{7}}
\newlabel{M-sec:exp_sim}{{\unhbox \voidb@x \hbox {V-A}}{7}}
\newlabel{M-eq:radar_manifold}{{24}{7}}
\newlabel{M-eq:radar_vandermonde}{{25}{7}}
\newlabel{M-eq:radar_equation}{{26}{7}}
\newlabel{M-fig:sim_gospa}{{4}{8}}
\newlabel{M-eq:mean_field}{{27}{8}}
\newlabel{M-sec:exp_radio}{{\unhbox \voidb@x \hbox {V-B}}{8}}
\newlabel{M-fig:sim_intensity_maps}{{5a}{9}}
\newlabel{M-sub@fig:sim_intensity_maps}{{(a)}{a}}
\newlabel{M-fig:sim_intensity_diff}{{5b}{9}}
\newlabel{M-sub@fig:sim_intensity_diff}{{(b)}{b}}
\newlabel{M-fig:sim_intensity}{{5}{9}}
\newlabel{M-fig:radar_camera}{{6a}{9}}
\newlabel{M-sub@fig:radar_camera}{{(a)}{a}}
\newlabel{M-fig:radar_spectrum}{{6b}{9}}
\newlabel{M-sub@fig:radar_spectrum}{{(b)}{b}}
\newlabel{M-fig:radar_xy}{{6c}{9}}
\newlabel{M-sub@fig:radar_xy}{{(c)}{c}}
\newlabel{M-fig:radar_results}{{6}{9}}
\newlabel{M-tab:performance_uwcr}{{II}{9}}
\newlabel{M-fig:radar_coverage}{{7a}{9}}
\newlabel{M-sub@fig:radar_coverage}{{(a)}{a}}
\newlabel{M-fig:radar_intensity}{{7b}{9}}
\newlabel{M-sub@fig:radar_intensity}{{(b)}{b}}
\newlabel{M-fig:coverage_intensity}{{7}{9}}
\newlabel{M-fig:sonar_s59}{{8a}{10}}
\newlabel{M-sub@fig:sonar_s59}{{(a)}{a}}
\newlabel{M-fig:sonar_est}{{8b}{10}}
\newlabel{M-sub@fig:sonar_est}{{(b)}{b}}
\newlabel{M-fig:sonar_panel}{{8}{10}}
\newlabel{M-eq:radar_visualization_context}{{28}{10}}
\newlabel{M-sec:exp_sonar}{{\unhbox \voidb@x \hbox {V-C}}{10}}
\newlabel{M-tab:performance_sonar}{{III}{11}}
\newlabel{M-fig:sonar_curves}{{9}{11}}
\newlabel{M-sec:latent_field_ablation}{{\unhbox \voidb@x \hbox {V-C}5}{12}}
\newlabel{M-sec:conclusion}{{VI}{12}}
\makeatother

